Foundations of Interpretable Models

We argue that existing definitions of interpretability are not actionable in that they fail to inform users about general, sound, and robust interpretable model design. This makes current interpretability research fundamentally ill-posed. To address this issue, we propose a definition of interpretability that is general, simple, and subsumes existing informal notions within the interpretable AI community. We show that our definition is actionable, as it directly reveals the foundational properties, underlying assumptions, principles, data structures, and architectural features necessary for designing interpretable models. Building on this, we propose a general blueprint for designing interpretable models and introduce the first open-sourced library with native support for interpretable data structures and processes.

==> tikz/tikzit_vertical.tex <==
% TiKZ style file generated by TikZiT. You may edit this file manually,
% but some things (e.g. comments) may be overwritten. To be readable in
% TikZiT, the only non-comment lines must be of the form:
% \tikzstyle{NAME}=[PROPERTY LIST]

% Node styles
\tikzstyle{none}=[]
\tikzstyle{white dot}=[fill=white, draw=black, shape=circle, text width=.1cm, inner sep=.03cm]
\tikzstyle{red dot}=[fill={rgb,255: red,163; green,0; blue,2}, draw=black, shape=circle]
\tikzstyle{medium box}=[fill=white, draw=black, shape=rectangle, minimum width=2cm, minimum height=1.cm]
\tikzstyle{small box}=[fill=white, draw=black, shape=rectangle, minimum width=.5cm, minimum height=.5cm]
\tikzstyle{triangle}=[fill=white, draw=black, regular polygon, regular polygon sides=3, shape border rotate=180, minimum width=1.cm, text width=.3cm, inner sep=.0cm, align=center, anchor=center]


% Edge styles
\tikzstyle{new edge style 0}=[-, fill=none, draw={rgb,255: red,0; green,172; blue,187}]
\tikzstyle{thick edge}=[-, line width=.03cm]


\pgfdeclarelayer{nodelayer}
\pgfdeclarelayer{edgelayer}
\pgfsetlayers{nodelayer,background,main,edgelayer}


\newcommand{\conceptProcess}{
\begin{tikzpicture}
	\begin{pgfonlayer}{nodelayer}
		\node [style=medium box] (5) at (-7, -4.75) {$f$};
		\node [style=none] (7) at (-7.75, -5.25) {};
		\node [style=none] (9) at (-6.25, -5.25) {};
		\node [style=none] (11) at (-7, -4.25) {};
		\node [style=none, label={above:$Y$}] (15) at (-7, -3.75) {};
		\node [style=none] (32) at (-7, -5.65) {$\dots$};
		\node [style=small box] (33) at (-7.75, -6) {$C_1$};
		\node [style=small box] (34) at (-6.25, -6) {$C_k$};
	\end{pgfonlayer}
	\begin{pgfonlayer}{edgelayer}
		\draw [in=-90, out=90, looseness=1.25] (11.center) to (15.center);
		\draw (7.center) to (33);
		\draw (9.center) to (34);
	\end{pgfonlayer}
\end{tikzpicture}
}

\newcommand{\conditionalProcess}{
\begin{tikzpicture}
	\begin{pgfonlayer}{nodelayer}
		\node [style=medium box] (5) at (-7, -4.75) {$P(C \mid X)$};
		\node [style=none] (9) at (-7, -5.25) {};
		\node [style=none] (11) at (-7, -4.25) {};
		\node [style=none, label={above:$C$}] (15) at (-7, -3.75) {};
		\node [style=small box] (34) at (-7, -6) {$X$};
	\end{pgfonlayer}
	\begin{pgfonlayer}{edgelayer}
		\draw [in=-90, out=90, looseness=1.25] (11.center) to (15.center);
		\draw (9.center) to (34);
	\end{pgfonlayer}
\end{tikzpicture}
}

\newcommand{\cbmProcess}{
\begin{tikzpicture}
	\begin{pgfonlayer}{nodelayer}
		\node [style=medium box] (5) at (-7, -4.75) {$P(C_1 \mid X)$};
		\node [style=none] (9) at (-7, -5.25) {};
		\node [style=none] (11) at (-7, -4.25) {};
		\node [style=none] (15) at (-6.5, -3.25) {};
		\node [style=medium box] (40) at (-4.5, -4.75) {$P(C_k \mid X)$};
		\node [style=none] (41) at (-4.5, -5.25) {};
		\node [style=none] (42) at (-4.5, -4.25) {};
		\node [style=none] (43) at (-5, -3.25) {};
		\node [style=small box] (44) at (-5.75, -6.5) {$X$};
		\node [style=white dot] (45) at (-5.75, -5.75) {};
		\node [style=none] (46) at (-5.75, -4.75) {$\dots$};
		\node [style=medium box] (47) at (-5.75, -2.75) {$P(Y \mid C_1, \dots,C_k)$};
		\node [style=none] (50) at (-5.75, -2.25) {};
		\node [style=none, label={above:$Y$}] (51) at (-5.75, -1.75) {};
		\node [style=none] (52) at (-7.25, -3.75) {$C_1$};
		\node [style=none] (53) at (-4.25, -3.75) {$C_k$};
	\end{pgfonlayer}
	\begin{pgfonlayer}{edgelayer}
		\draw [in=-90, out=90, looseness=1.25] (11.center) to (15.center);
		\draw [in=-90, out=90, looseness=1.25] (42.center) to (43.center);
		\draw (44) to (45);
		\draw [bend right=45] (9.center) to (41.center);
		\draw [in=-90, out=90, looseness=1.25] (50.center) to (51.center);
	\end{pgfonlayer}
\end{tikzpicture}
}

\newcommand{\compositionalElements}{
\begin{tikzpicture}
	\begin{pgfonlayer}{nodelayer}
		\node [style=medium box] (5) at (-7, -4.75) {$f$};
		\node [style=none] (7) at (-7.75, -5.25) {};
		\node [style=none] (9) at (-6.25, -5.25) {};
		\node [style=none] (11) at (-7, -4.25) {};
		\node [style=none] (12) at (-7.75, -6) {};
		\node [style=none] (14) at (-6.25, -6) {};
		\node [style=none] (15) at (-7, -3.5) {};
		\node [style=white dot] (16) at (-3, -4.75) {};
		\node [style=none] (17) at (-3, -5.5) {};
		\node [style=none] (18) at (-3.75, -4) {};
		\node [style=none] (19) at (-2.25, -4) {};
		\node [style=none] (20) at (0.75, -4.5) {};
		\node [style=none] (21) at (0.75, -5.5) {};
		\node [style=none] (22) at (1.125, -4.5) {};
		\node [style=none] (23) at (0.375, -4.5) {};
		\node [style=none] (24) at (1, -4.375) {};
		\node [style=none] (25) at (0.5, -4.375) {};
		\node [style=none] (26) at (0.875, -4.25) {};
		\node [style=none] (27) at (0.625, -4.25) {};
		\node [style=none] (32) at (-7, -5.9) {$\dots$};
		\node [style=triangle] (33) at (3.625, -5.25) {$k$};
		\node [style=none] (34) at (3.625, -5) {};
		\node [style=none] (35) at (3.625, -4.25) {};
		\node [style=none] (37) at (5.875, -5.25) {};
		\node [style=none] (38) at (7.375, -5.25) {};
	\end{pgfonlayer}
	\begin{pgfonlayer}{edgelayer}
		\draw (12.center) to (7.center);
		\draw (14.center) to (9.center);
		\draw [in=-90, out=90, looseness=1.25] (11.center) to (15.center);
		\draw (17.center) to (16);
		\draw [bend right=90, looseness=1.75] (18.center) to (19.center);
		\draw (21.center) to (20.center);
		\draw [style=thick edge] (23.center) to (22.center);
		\draw [style=thick edge] (25.center) to (24.center);
		\draw [style=thick edge] (27.center) to (26.center);
		\draw [in=-90, out=90, looseness=1.25] (34.center) to (35.center);
		\draw [bend left=90, looseness=2.00] (37.center) to (38.center);
	\end{pgfonlayer}
\end{tikzpicture}

}

\newcommand{\compositionalExample}{
\begin{tikzpicture}
	\begin{pgfonlayer}{nodelayer}
		\node [style=medium box] (42) at (-7, -1.25) {$C_1 \vee C_4$};
		\node [style=none] (45) at (-7, -0.75) {};
		\node [style=none, label={above:$Y$}] (46) at (-7, -0.5) {};
		\node [style=medium box] (47) at (-5.25, -3.25) {$\neg C_2 \wedge C_{3}$};
		\node [style=none] (49) at (-6.5, -1.75) {};
		\node [style=none] (52) at (-5.25, -2.75) {};
		\node [style=none, label={right:$C_4$}] (53) at (-5.5, -2.25) {};
		\node [style=medium box] (54) at (-9, -4.75) {$P(C_1 \mid X)$};
		\node [style=none] (55) at (-9, -5.25) {};
		\node [style=medium box] (57) at (-6.5, -4.75) {$P(C_2 \mid X)$};
		\node [style=none] (58) at (-6.5, -5.25) {};
		\node [style=none] (59) at (-6.5, -4.25) {};
		\node [style=small box] (60) at (-6.5, -6.25) {$X$};
		\node [style=white dot] (61) at (-6.5, -5.75) {};
		\node [style=none] (63) at (-7.5, -1.75) {};
		\node [style=medium box] (66) at (-4, -4.75) {$P(C_3 \mid X)$};
		\node [style=none] (67) at (-4, -5.25) {};
		\node [style=none] (68) at (-4, -4.25) {};
		\node [style=none] (69) at (-5.75, -3.75) {};
		\node [style=none] (71) at (-4.75, -3.75) {};
		\node [style=none] (74) at (-18.5, -3.5) {};
		\node [style=medium box] (75) at (-16, -1.75) {$C_1 \vee (\neg C_2 \wedge C_3)$};
		\node [style=none] (76) at (-16, -1.25) {};
		\node [style=none, label={above:$Y$}] (77) at (-16, -0.75) {};
		\node [style=medium box] (78) at (-18.5, -4) {$P(C_1 \mid X)$};
		\node [style=none] (79) at (-18.5, -4.5) {};
		\node [style=none] (80) at (-18.5, -3.5) {};
		\node [style=medium box] (81) at (-16, -4) {$P(C_2 \mid X)$};
		\node [style=none] (82) at (-16, -4.5) {};
		\node [style=none] (83) at (-16, -3.5) {};
		\node [style=small box] (84) at (-16, -6) {$X$};
		\node [style=white dot] (85) at (-16, -5.25) {};
		\node [style=medium box] (86) at (-13.5, -4) {$P(C_3 \mid X)$};
		\node [style=none] (87) at (-13.5, -4.5) {};
		\node [style=none] (88) at (-13.5, -3.5) {};
		\node [style=none] (89) at (-16.5, -2.25) {};
		\node [style=none] (90) at (-16, -2.25) {};
		\node [style=none] (91) at (-15.5, -2.25) {};
		\node [style=none, label={right:{\Huge$\equiv$}}] (92) at (-11.75, -4) {};
		\node [style=none] (93) at (-9, -4.25) {};
	\end{pgfonlayer}
	\begin{pgfonlayer}{edgelayer}
		\draw (45.center) to (46.center);
		\draw [in=-90, out=90, looseness=0.75] (52.center) to (49.center);
		\draw (60) to (61);
		\draw [bend right=15, looseness=0.75] (55.center) to (61);
		\draw (58.center) to (61);
		\draw [bend right=15, looseness=0.75] (61) to (67.center);
		\draw (76.center) to (77.center);
		\draw (84) to (85);
		\draw [bend right=15, looseness=0.75] (79.center) to (85);
		\draw (82.center) to (85);
		\draw [bend right=15, looseness=0.75] (85) to (87.center);
		\draw [in=-90, out=90, looseness=0.50] (80.center) to (89.center);
		\draw (83.center) to (90.center);
		\draw [in=-90, out=90, looseness=0.50] (88.center) to (91.center);
		\draw [in=-90, out=90, looseness=0.75] (93.center) to (63.center);
		\draw [in=-90, out=90, looseness=0.75] (59.center) to (69.center);
		\draw [in=-90, out=90, looseness=0.75] (68.center) to (71.center);
	\end{pgfonlayer}
\end{tikzpicture}
}


% \newcommand{\dointerventionExample}{
% \begin{tikzpicture}
% 	\begin{pgfonlayer}{nodelayer}
% 		\node [style=medium box] (5) at (-7, -4.5) {$C_1 \vee C_{3}$};
% 		\node [style=none] (7) at (-7.75, -5) {};
% 		\node [style=none] (11) at (-7, -4) {};
% 		\node [style=small box] (12) at (-9.75, -6.25) {$C_1$};
% 		\node [style=none] (15) at (-7, -4) {};
% 		\node [style=white dot] (16) at (-7, -3.25) {};
% 		\node [style=none] (17) at (-7, -4) {};
% 		\node [style=none, label={above:$Y_1$}] (18) at (-8, 0.25) {};
% 		\node [style=none] (19) at (-5.75, -2.75) {};
% 		\node [style=none] (20) at (-7.25, -5.75) {};
% 		\node [style=small box] (21) at (-7.25, -6.25) {$C_2$};
% 		\node [style=none] (22) at (-6.875, -5.75) {};
% 		\node [style=none] (23) at (-7.625, -5.75) {};
% 		\node [style=none] (24) at (-7, -5.625) {};
% 		\node [style=none] (25) at (-7.5, -5.625) {};
% 		\node [style=none] (26) at (-7.125, -5.5) {};
% 		\node [style=none] (27) at (-7.375, -5.5) {};
% 		\node [style=none] (37) at (-6.25, -5) {};
% 		\node [style=small box] (38) at (-5.125, -6.25) {$C_3$};
% 		\node [style=medium box] (42) at (-5.25, -0.75) {$Y_1 \wedge \neg Y_{2}$};
% 		\node [style=small box] (43) at (-2.5, -6.25) {$C_4$};
% 		\node [style=none] (44) at (-3, -5) {};
% 		\node [style=none] (45) at (-5.25, -0.25) {};
% 		\node [style=none, label={above:$Y_3$}] (46) at (-5.25, 0.25) {};
% 		\node [style=medium box] (47) at (-3.5, -4.5) {$C_3 \wedge C_{4}$};
% 		\node [style=none] (48) at (-4, -5) {};
% 		\node [style=none] (49) at (-4.75, -1.25) {};
% 		\node [style=white dot] (51) at (-5.125, -5.5) {};
% 		\node [style=none] (52) at (-3.5, -4) {};
% 		\node [style=none, label={right:$Y_2$}] (53) at (-3.75, -3.25) {};
% 		\node [style=none] (54) at (-5.75, -2.75) {};
% 		\node [style=none] (55) at (-5.375, -2.75) {};
% 		\node [style=none] (56) at (-6.125, -2.75) {};
% 		\node [style=none] (57) at (-5.5, -2.625) {};
% 		\node [style=none] (58) at (-6, -2.625) {};
% 		\node [style=none] (59) at (-5.625, -2.5) {};
% 		\node [style=none] (60) at (-5.875, -2.5) {};
% 		\node [style=triangle] (61) at (-5.75, -1.75) {$y_1$};
% 		\node [style=none] (62) at (-5.75, -1.25) {};
% 	\end{pgfonlayer}
% 	\begin{pgfonlayer}{edgelayer}
% 		\draw [in=-90, out=90] (12) to (7.center);
% 		\draw [in=-90, out=90, looseness=1.25] (11.center) to (15.center);
% 		\draw (17.center) to (16);
% 		\draw (21) to (20.center);
% 		\draw [style=thick edge] (23.center) to (22.center);
% 		\draw [style=thick edge] (25.center) to (24.center);
% 		\draw [style=thick edge] (27.center) to (26.center);
% 		\draw [in=150, out=-90] (18.center) to (16);
% 		\draw [in=-90, out=0] (16) to (19.center);
% 		\draw [in=-90, out=90, looseness=0.75] (43) to (44.center);
% 		\draw (45.center) to (46.center);
% 		\draw (38) to (51);
% 		\draw [in=-90, out=180, looseness=0.75] (51) to (37.center);
% 		\draw [in=-90, out=0] (51) to (48.center);
% 		\draw [in=-90, out=90] (52.center) to (49.center);
% 		\draw [style=thick edge] (56.center) to (55.center);
% 		\draw [style=thick edge] (58.center) to (57.center);
% 		\draw [style=thick edge] (60.center) to (59.center);
% 		\draw (61) to (62.center);
% 	\end{pgfonlayer}
% \end{tikzpicture}
% }

\newcommand{\expressivityParametricJoint}{
\begin{tikzpicture}
	\begin{pgfonlayer}{nodelayer}
		\node [style=medium box] (5) at (-7, -4.25) {$P(C \mid X)$};
		\node [style=none] (9) at (-7, -4.75) {};
		\node [style=none] (11) at (-7, -3.75) {};
		\node [style=none] (15) at (-6.5, -3.25) {};
		\node [style=none] (42) at (-4.5, -4) {};
		\node [style=none] (43) at (-5, -3.25) {};
		\node [style=small box] (44) at (-7, -5.25) {$X$};
		\node [style=medium box] (47) at (-5.75, -2.75) {$P(Y \mid C; \theta)$};
		\node [style=none] (50) at (-5.75, -2.25) {};
		\node [style=none, label={above:$Y$}] (51) at (-5.75, -2) {};
		\node [style=small box] (54) at (-4.5, -4.25) {$\theta$};
	\end{pgfonlayer}
	\begin{pgfonlayer}{edgelayer}
		\draw [in=-90, out=90, looseness=1.25] (11.center) to (15.center);
		\draw [in=-90, out=90, looseness=1.50] (42.center) to (43.center);
		\draw [in=-90, out=90, looseness=1.25] (50.center) to (51.center);
		\draw (44) to (9.center);
	\end{pgfonlayer}
\end{tikzpicture}
}

\newcommand{\expressivityDCR}{
\begin{tikzpicture}
	\begin{pgfonlayer}{nodelayer}
		\node [style=medium box] (5) at (-7, -4.25) {$P(C \mid X)$};
		\node [style=none] (9) at (-7, -4.75) {};
		\node [style=none] (11) at (-7, -3.75) {};
		\node [style=none] (15) at (-6.5, -3.25) {};
		\node [style=medium box] (40) at (-4.5, -4.25) {$P(\theta \mid X)$};
		\node [style=none] (41) at (-4.5, -4.75) {};
		\node [style=none] (42) at (-4.5, -3.75) {};
		\node [style=none] (43) at (-5, -3.25) {};
		\node [style=small box] (44) at (-5.75, -6) {$X$};
		\node [style=white dot] (45) at (-5.75, -5.25) {};
		\node [style=medium box] (47) at (-5.75, -2.75) {$P(Y \mid C; \theta)$};
		\node [style=none] (50) at (-5.75, -2.25) {};
		\node [style=none, label={above:$Y$}] (51) at (-5.75, -2) {};
	\end{pgfonlayer}
	\begin{pgfonlayer}{edgelayer}
		\draw [in=-90, out=90, looseness=1.25] (11.center) to (15.center);
		\draw [in=-90, out=90, looseness=1.25] (42.center) to (43.center);
		\draw (44) to (45);
		\draw [bend right=45] (9.center) to (41.center);
		\draw [in=-90, out=90, looseness=1.25] (50.center) to (51.center);
	\end{pgfonlayer}
\end{tikzpicture}
}


\newcommand{\expressivityCMR}{
\begin{tikzpicture}
	\begin{pgfonlayer}{nodelayer}
		\node [style=medium box] (5) at (-7.75, -6) {$P(C \mid X)$};
		\node [style=none] (9) at (-7.75, -6.5) {};
		\node [style=none] (11) at (-7.75, -5.5) {};
		\node [style=none] (15) at (-6.25, -3.25) {};
		\node [style=medium box] (40) at (-5.25, -6) {$P(S \mid X)$};
		\node [style=none] (41) at (-5.25, -6.5) {};
		\node [style=none] (42) at (-4.5, -4) {};
		\node [style=none] (43) at (-5.25, -3.25) {};
		\node [style=small box] (44) at (-6.5, -7.75) {$X$};
		\node [style=white dot] (45) at (-6.5, -7) {};
		\node [style=medium box] (47) at (-5.75, -2.75) {$P(Y \mid C; \theta)$};
		\node [style=none] (50) at (-5.75, -2.25) {};
		\node [style=none, label={above:$Y$}] (51) at (-5.75, -2) {};
		\node [style=small box] (52) at (-4, -7.75) {$M_\Theta$};
		\node [style=medium box] (53) at (-4.5, -4.5) {$P(\theta \mid S, M_\Theta)$};
		\node [style=none] (54) at (-4, -7.5) {};
		\node [style=none] (55) at (-4, -5) {};
		\node [style=none] (56) at (-5.25, -5.5) {};
		\node [style=none] (57) at (-5, -5) {};
	\end{pgfonlayer}
	\begin{pgfonlayer}{edgelayer}
		\draw [in=-90, out=90, looseness=1.25] (11.center) to (15.center);
		\draw [in=-90, out=90, looseness=1.25] (42.center) to (43.center);
		\draw (44) to (45);
		\draw [bend right=45] (9.center) to (41.center);
		\draw [in=-90, out=90, looseness=1.25] (50.center) to (51.center);
		\draw [in=-90, out=90, looseness=1.25] (54.center) to (55.center);
		\draw [in=-90, out=90, looseness=1.25] (56.center) to (57.center);
	\end{pgfonlayer}
\end{tikzpicture}
}


\newcommand{\dointerventionExample}{
\begin{tikzpicture}
	\begin{pgfonlayer}{nodelayer}
		\node [style=none] (19) at (-5, -2.75) {};
		\node [style=medium box] (42) at (-4.5, -0.75) {$P(Y \mid C)$};
		\node [style=none] (45) at (-4.5, -0.25) {};
		\node [style=none, label={above:$Y$}] (46) at (-4.5, 0) {};
		\node [style=none] (49) at (-4, -1.25) {};
		\node [style=none] (54) at (-5, -2.75) {};
		\node [style=none] (55) at (-4.625, -2.75) {};
		\node [style=none] (56) at (-5.375, -2.75) {};
		\node [style=none] (57) at (-4.75, -2.625) {};
		\node [style=none] (58) at (-5.25, -2.625) {};
		\node [style=none] (59) at (-4.875, -2.5) {};
		\node [style=none] (60) at (-5.125, -2.5) {};
		\node [style=triangle] (61) at (-5, -1.75) {$k$};
		\node [style=none] (62) at (-5, -1.25) {};
		\node [style=medium box] (63) at (-5.75, -3.75) {$P(C_1 \mid X)$};
		\node [style=none] (64) at (-5.75, -4.25) {};
		\node [style=none] (65) at (-5.75, -3.25) {};
		\node [style=medium box] (66) at (-3.25, -3.75) {$P(C_k \mid X)$};
		\node [style=none] (67) at (-3.25, -4.25) {};
		\node [style=none] (68) at (-3.25, -3.25) {};
		\node [style=small box] (69) at (-4.5, -5.25) {$X$};
		\node [style=white dot] (70) at (-4.5, -4.75) {};
		\node [style=none] (71) at (-4.5, -3.75) {$\dots$};
	\end{pgfonlayer}
	\begin{pgfonlayer}{edgelayer}
		\draw (45.center) to (46.center);
		\draw [style=thick edge] (56.center) to (55.center);
		\draw [style=thick edge] (58.center) to (57.center);
		\draw [style=thick edge] (60.center) to (59.center);
		\draw (61) to (62.center);
		\draw (69) to (70);
		\draw [bend right=45] (64.center) to (67.center);
		\draw [in=-90, out=90, looseness=0.75] (65.center) to (54.center);
		\draw [in=-90, out=90] (68.center) to (49.center);
	\end{pgfonlayer}
\end{tikzpicture}
}


\newcommand{\gtinterventionExample}{
\begin{tikzpicture}
	\begin{pgfonlayer}{nodelayer}
		\node [style=none] (19) at (-5, -2.75) {};
		\node [style=medium box] (42) at (-4.5, -0.75) {$P(Y \mid C)$};
		\node [style=none] (45) at (-4.5, -0.25) {};
		\node [style=none, label={above:$Y$}] (46) at (-4.5, 0) {};
		\node [style=none] (49) at (-4, -1.25) {};
		\node [style=none] (54) at (-5, -2.75) {};
		\node [style=none] (55) at (-4.625, -2.75) {};
		\node [style=none] (56) at (-5.375, -2.75) {};
		\node [style=none] (57) at (-4.75, -2.625) {};
		\node [style=none] (58) at (-5.25, -2.625) {};
		\node [style=none] (59) at (-4.875, -2.5) {};
		\node [style=none] (60) at (-5.125, -2.5) {};
		\node [style=small box] (61) at (-5, -1.75) {$C_1$};
		\node [style=none] (62) at (-5, -1.25) {};
		\node [style=medium box] (63) at (-5.75, -3.75) {$P(C_1 \mid X)$};
		\node [style=none] (64) at (-5.75, -4.25) {};
		\node [style=none] (65) at (-5.75, -3.25) {};
		\node [style=medium box] (66) at (-3.25, -3.75) {$P(C_k \mid X)$};
		\node [style=none] (67) at (-3.25, -4.25) {};
		\node [style=none] (68) at (-3.25, -3.25) {};
		\node [style=small box] (69) at (-4.5, -5.25) {$X$};
		\node [style=white dot] (70) at (-4.5, -4.75) {};
		\node [style=none] (71) at (-4.5, -3.75) {$\dots$};
	\end{pgfonlayer}
	\begin{pgfonlayer}{edgelayer}
		\draw (45.center) to (46.center);
		\draw [style=thick edge] (56.center) to (55.center);
		\draw [style=thick edge] (58.center) to (57.center);
		\draw [style=thick edge] (60.center) to (59.center);
		\draw (61) to (62.center);
		\draw (69) to (70);
		\draw [bend right=45] (64.center) to (67.center);
		\draw [in=-90, out=90, looseness=0.75] (65.center) to (54.center);
		\draw [in=-90, out=90] (68.center) to (49.center);
	\end{pgfonlayer}
\end{tikzpicture}
}

\newcommand{\alignmentProcess}{
\begin{tikzpicture}
	\begin{pgfonlayer}{nodelayer}
		\node [style=medium box] (5) at (-7, -4.25) {$P(C_i \mid X)$};
		\node [style=none] (9) at (-7, -4.75) {};
		\node [style=none] (11) at (-7, -3.75) {};
		\node [style=none] (15) at (-6.5, -3.25) {};
		\node [style=medium box] (40) at (-4.5, -4.25) {$P(C_j^h \mid X)$};
		\node [style=none] (41) at (-4.5, -4.75) {};
		\node [style=none] (42) at (-4.5, -3.75) {};
		\node [style=none] (43) at (-5, -3.25) {};
		\node [style=small box] (44) at (-5.75, -5.75) {$X$};
		\node [style=white dot] (45) at (-5.75, -5.25) {};
		\node [style=medium box] (47) at (-5.75, -2.75) {$\Lambda(C_i, C_j^h)$};
		\node [style=none] (50) at (-5.75, -2.25) {};
		\node [style=none, label={above:$\eta$}] (51) at (-5.75, -2) {};
	\end{pgfonlayer}
	\begin{pgfonlayer}{edgelayer}
		\draw [in=-90, out=90, looseness=1.25] (11.center) to (15.center);
		\draw [in=-90, out=90, looseness=1.25] (42.center) to (43.center);
		\draw (44) to (45);
		\draw [bend right=45] (9.center) to (41.center);
		\draw [in=-90, out=90, looseness=1.25] (50.center) to (51.center);
	\end{pgfonlayer}
\end{tikzpicture}
}

\newcommand{\alignmentProcessLoss}{
\begin{tikzpicture}
	\begin{pgfonlayer}{nodelayer}
		\node [style=medium box] (5) at (-7, -4.25) {$P(C_i \mid X; \theta_c)$};
		\node [style=none] (9) at (-6.5, -4.75) {};
		\node [style=none] (11) at (-7, -3.75) {};
		\node [style=none] (15) at (-6.5, -3.25) {};
		\node [style=medium box] (40) at (-4.5, -4.25) {$P(C_j^h \mid X)$};
		\node [style=none] (41) at (-4.5, -4.75) {};
		\node [style=none] (42) at (-4.5, -3.75) {};
		\node [style=none] (43) at (-5, -3.25) {};
		\node [style=small box] (44) at (-5.5, -5.675) {$X$};
		\node [style=white dot] (45) at (-5.5, -5.175) {};
		\node [style=medium box] (47) at (-5.75, -2.75) {$\Lambda(C_i, C_j^h)$};
		\node [style=none] (53) at (-7.5, -4.75) {};
		\node [style=none] (54) at (-8.25, -0.25) {};
		\node [style=none] (56) at (-10.25, -3) {};
		\node [style=none, label={below:$\theta_c$}] (58) at (-9.5, -5.75) {};
		\node [style=medium box] (59) at (-6.75, -1.25) {$P(\theta_c \mid \eta, \theta_c)$};
		\node [style=none] (60) at (-5.75, -2.25) {};
		\node [style=none] (61) at (-6.25, -1.75) {};
		\node [style=none] (63) at (-7.25, -1.75) {};
		\node [style=white dot] (66) at (-9, -5.175) {};
	\end{pgfonlayer}
	\begin{pgfonlayer}{edgelayer}
		\draw [in=-90, out=90, looseness=1.25] (11.center) to (15.center);
		\draw [in=-90, out=90, looseness=1.25] (42.center) to (43.center);
		\draw (44) to (45);
		\draw [bend right=45] (9.center) to (41.center);
		\draw [in=90, out=-180, looseness=1.25] (54.center) to (56.center);
		\draw [in=90, out=0] (54.center) to (59);
		\draw [in=-90, out=90, looseness=1.25] (60.center) to (61.center);
		\draw [in=-90, out=0, looseness=0.75] (66) to (53.center);
		\draw [in=-90, out=90, looseness=1.25] (66) to (63.center);
		\draw [in=-180, out=-90, looseness=0.75] (56.center) to (58.center);
		\draw [in=-90, out=0, looseness=1.25] (58.center) to (66);
	\end{pgfonlayer}
\end{tikzpicture}
}
